Coswara: A respiratory sounds and symptoms dataset for remote screening of SARS-CoV-2 infection

This paper presents the Coswara dataset, a dataset containing diverse set of respiratory sounds and rich meta-data, recorded between April-2020 and February-2022 from 2635 individuals (1819 SARS-CoV-2 negative, 674 positive, and 142 recovered subjects). The respiratory sounds contained nine sound categories associated with variants of breathing, cough and speech. The rich metadata contained demographic information associated with age, gender and geographic location, as well as the health information relating to the symptoms, pre-existing respiratory ailments, comorbidity and SARS-CoV-2 test status. Our study is the first of its kind to manually annotate the audio quality of the entire dataset (amounting to 65~hours) through manual listening. The paper summarizes the data collection procedure, demographic, symptoms and audio data information. A COVID-19 classifier based on bi-directional long short-term (BLSTM) architecture, is trained and evaluated on the different population sub-groups contained in the dataset to understand the bias/fairness of the model. This enabled the analysis of the impact of gender, geographic location, date of recording, and language proficiency on the COVID-19 detection performance.

==> cls_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{p{5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}}
\hline
 & \multicolumn{2}{c}{\textbf{test1}} & \multicolumn{2}{c}{\textbf{test2}} & \multicolumn{2}{c}{\textbf{combined test}} \\ \cline{2-7} 
\multirow{-2}{*}{\textbf{Modality}} & \multicolumn{1}{c}{AUC} & Sens & \multicolumn{1}{c}{AUC} & Sens & \multicolumn{1}{c}{AUC} & Sens \\ \hline
\cellcolor[HTML]{EFEFEF}breathing-deep & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}74.3} & \cellcolor[HTML]{EFEFEF}36.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}77.2} & \cellcolor[HTML]{EFEFEF}36.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}75.7} & \cellcolor[HTML]{EFEFEF}34.0 \\ \hline
breathing-shallow & \multicolumn{1}{c}{77.4} & 28.0 & \multicolumn{1}{c}{78.9} & 28.0 & \multicolumn{1}{c}{77.9} & 28.0 \\ \hline
\cellcolor[HTML]{EFEFEF}cough-heavy & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}79.0} & \cellcolor[HTML]{EFEFEF}32.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}80.3} & \cellcolor[HTML]{EFEFEF}30.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}79.8} & \cellcolor[HTML]{EFEFEF}32.0 \\ \hline
cough-shallow & \multicolumn{1}{c}{76.5} & 36.0 & \multicolumn{1}{c}{76.3} & 32.0 & \multicolumn{1}{c}{76.6} & 38.0 \\ \hline
\cellcolor[HTML]{EFEFEF}counting-fast & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}78.9} & \cellcolor[HTML]{EFEFEF}38.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}81.2} & \cellcolor[HTML]{EFEFEF}28.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}79.4} & \cellcolor[HTML]{EFEFEF}36.0 \\ \hline
counting-normal & \multicolumn{1}{c}{80.7} & 36.0 & \multicolumn{1}{c}{81.5} & 38.0 & \multicolumn{1}{c}{80.8} & 31.0 \\ \hline
\cellcolor[HTML]{EFEFEF}vowel-a & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}77.1} & \cellcolor[HTML]{EFEFEF}20.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}82.0} & \cellcolor[HTML]{EFEFEF}38.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}79.3} & \cellcolor[HTML]{EFEFEF}28.0 \\ \hline
vowel-e & \multicolumn{1}{c}{75.9} & 36.0 & \multicolumn{1}{c}{79.0} & 34.0 & \multicolumn{1}{c}{77.3} & 33.0 \\ \hline
\cellcolor[HTML]{EFEFEF}vowel-o & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}71.8} & \cellcolor[HTML]{EFEFEF}32.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}75.3} & \cellcolor[HTML]{EFEFEF}24.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}73.6} & \cellcolor[HTML]{EFEFEF}22.0 \\ \hline
audio fusion & \multicolumn{1}{c}{83.7} & 58.0 & \multicolumn{1}{c}{85.2} & 38.0 & \multicolumn{1}{c}{84.1} & 38.0 \\ \hline
symptoms & \multicolumn{1}{c}{81.1} & 42.0 & \multicolumn{1}{c}{88.8} & 36.0 & \multicolumn{1}{c}{84.9} & 53.0 \\ \hline
\cellcolor[HTML]{EFEFEF}fusion & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}88.3} & \cellcolor[HTML]{EFEFEF}58.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}89.1} & \cellcolor[HTML]{EFEFEF}50.0 & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}88.1} & \cellcolor[HTML]{EFEFEF}47.0 \\ \hline
\end{tabular}
\caption{Classifier performance on test1, test2 and test\_combined set of ten modalities and their fusion.}
\label{tab:cls_result}
\end{table*}

==> table_annotation.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{llccc}
\hline
\textbf{Sound Category} & \textbf{} & \textbf{Excellent} & \textbf{Good} & \textbf{Bad} \\ \cline{1-1} \cline{3-5} 
breathing-shallow       &           & 72.4               & 11.3          & 16.3         \\
breathing-deep          &           & 73.5               & 12.2          & 14.3         \\
cough-shallow           &           & 82.8               & 11.1          & 6.1          \\
cough-heavy             &           & 86.3               & 7.5           & 6.2          \\
vowel-{[}u{]}           &           & 67.2               & 21.1          & 11.7         \\
vowel-{[}i{]}           &           & 80.4               & 10.8          & 8.8          \\
vowel-{[}ae{]}          &           & 77.6               & 14.2          & 8.2          \\
counting-normal         &           & 83.5               & 8.9           & 7.6          \\
counting-fast           &           & 84.2               & 7.8           & 8.0          \\ \cline{1-1} \cline{3-5} 
overall                 &           & 78.6               & 11.7          & 9.7          \\ \hline
\end{tabular}
\caption{Statistics of audio quality annotation after manual listening (all numbers are in $\%$)}
\label{tab:annotation_statistics}
\end{table}

==> table_bias_perfm.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{@{}llrlrlr@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Subset\\ from test set\end{tabular}} &  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Count\\ COVID/\\ Non-COVID\end{tabular}}} &  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}AUC\\ (\%)\end{tabular}}} &  & \multicolumn{1}{l}{\textbf{p value}} \\ \midrule
\textbf{Gender} &  & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} \\
Male &  & 54/218 &  & 93.0 (90.0-95.5) &  & 0.870 \\
Female &  & 46/82 &  & 91.2 (86.6-95.3) &  & 0.745 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Age} &  &  &  &  &  &  \\
15-30 &  & 40/145 &  & 91.0 (87.1-94.7) &  & 0.260 \\
30-45 &  & 22/93 &  & 89.9 (82.2-95.8) &  & 0.387 \\
45-60 &  & 22/35 &  & 96.1 (92.2-99.4) &  & 0.579 \\
60-95 &  & 8/6 &  & 86.0 (65.0-100.0) &  & 0.152 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Vaccination} &  &  &  &  &  &  \\
With &  & 67/58 &  & 86.9 (81.7-91.7) &  & p<0.050 \\
Without &  & 33/242 &  & 90.1 (84.7-94.5) &  & 0.260 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Mask} &  &  &  &  &  &  \\
With &  & 47/36 &  & 83.3 (75.9-90.1) &  & p<0.050 \\
Without &  & 53/94 &  & 87.1 (81.9, 91.9) &  & 0.397 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{English Proficiency} &  &  &  &  &  &  \\
With &  & 91/289 &  & 92.0 (89.2-94.6) &  &  0.904 \\
Without &  & 9/11 &  & 88.8 (73.7-100.0) &  & 0.471\\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Date of collection} &  &  &  &  &  &  \\
Before Dec. 21 &  & 50/150 &  & 91.9 (87.7-95.2) &  & 0.110 \\
After Dec. 21 &  & 50/150 &  & 92.9 (89.3-95.9) &  & 0.110 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Collection Province} &  &  &  &  &  &  \\
Karnataka &  & 52/99 &  & 95.5 (92.3-98.3) &  & 0.402 \\
Others &  & 48/201 &  & 92.0 (89.3-94.4) &  & 0.509 \\

% \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7}
% \textbf{COVID severity and illness} &  &  &  &  &  &  \\
% Pos-moderate vs healthy &  & 18/243 &  & 99.1 (98.0-99.9) &  & p<0.050 \\
% Pos-moderate vs symp. &  & 18/32 &  & 67.1 (53.6-80.0) &  & p<0.050 \\
% Pos-moderate vs resp. ail. &  & 18/25 &  & 87.8 (79.3-95.1) &  & 0.112 \\
% Pos-mild vs healthy &  & 66/243 &  & 98.7 (97.6-99.6) &  & p<0.050 \\
% Pos-mild vs symp. &  & 66/32 &  & 72.8 (63.2-82.2) &  & p<0.050 \\
% Pos-mild vs resp. ail. &  & 66/25 &  & 89.9 (83.2-95.2) &  & 0.088 \\
% Pos-asymp vs healthy &  & 16/243 &  & 83.0 (73.6-92.0) &  & p<0.005 \\
% Pos-asymp vs symp. &  & 16/32 &  & 32.6 (18.4-47.1) &  & p<0.050 \\
% Pos-asymp vs resp. ail. &  & 16/25 &  & 63.1 (48.8-77.6) &  & p<0.050 \\
\cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7}
\textbf{Prevalence} &  &  &  &  &  &  \\
20\% &  & 70/280 &  & 92.0 (90.7-93.3) &  & 0.781 \\
10\% &  & 30/270 &  & 91.7 (87.5-95.9) &  & 0.357 \\
5\% &  & 15/285 &  & 91.4 (85.0-97.8) &  & 0.523 \\
2.5\% &  & 7/273 &  & 92.2 (81.8-100.0) &  & 0.588 \\ \bottomrule
\end{tabular}

\caption{Description of the subject categories used in analysis, and the AUC performance obtained using the BLSTM classifier. The p-values correspond to the t-test performed between scores from the full test set and the ones from the population sub-group considered.}
\label{tab:bias_analysis}
\vspace{-0.2in}
\end{table}

==> table_bias_perfm_p_val.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}
{
\begin{tabular}{@{}llrlrlr@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Subset\\ from test set\end{tabular}} &  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Count\\ COVID/\\ Non-COVID\end{tabular}}} &  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}AUC\\ (\%)\end{tabular}}} &  & \multicolumn{1}{l}{\textbf{p value}} \\ \midrule
\textbf{Gender} &  & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} \\
Male &  & 54/218 &  & 93.0 (90.0-95.5) &  & 6.823e-23 \\
Female &  & 46/82 &  & 91.2 (86.6-95.3) &  & 7.362e-15 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Age} &  &  &  &  &  &  \\
15-30 &  & 40/145 &  & 91.0 (87.1-94.7) &  & 1.131e-15 \\
30-45 &  & 22/93 &  & 89.9 (82.2-95.8) &  & 3.341e-09 \\
45-60 &  & 22/35 &  & 96.1 (92.2-99.4) &  & 3.106e-09 \\
60-95 &  & 8/6 &  & 86.0 (65.0-100.0) &  & 0.017 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Vaccination} &  &  &  &  &  &  \\
With &  & 67/58 &  & 90.1 (84.7-94.5) &  & 7.116e-13 \\
Without &  & 33/242 &  & 90.2 &  & 3.539e-14 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Mask} &  &  &  &  &  &  \\
With &  & 47/36 &  & 83.2 &  & 1.239e-07 \\
Without &  & 53/94 &  & 87.0 &  & 5.307e-14 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{English Proficiency} &  &  &  &  &  &  \\
With &  & 91/289 &  & 92.0 (89.2-94.6) &  &  5.056e-34 \\
Without &  & 9/11 &  & 88.8 (73.7-100.0) &  & 0.002\\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Date of collection} &  &  &  &  &  &  \\
Before Dec. 21 &  & 50/150 &  & 91.9 (87.7-95.2) &  & 2.936e-19 \\
After Dec. 21 &  & 50/150 &  & 92.9 (89.3-95.9) &  & 5.398e-20 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{Collection Province} &  &  &  &  &  &  \\
Karnataka &  & 52/99 &  & 95.4 &  & 2.748e-20 \\
Tamil Nadu &  & 29/28 &  & 85.7 &  & 1.908e-06 \\
Kerala &  & 3/9 &  & 100.0 &  & 0.008 \\
Maharashtra &  & 9/31 &  & 76.0 &  & 0.01 \\
Others &  & 7/133 &  & 85.4 &  & 8.288e-04 \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7} 
\textbf{COVID severity and illness} &  &  &  &  &  &  \\
moderate vs healthy &  & 18/275 &  & 95.5 &  & 5.153e-11 \\
moderate vs resp. ail. &  & 18/25 &  & 85.7 &  & 1.908e-06 \\
mild vs healthy &  & 66/275 &  & 95.7 &  & 4.817e-31 \\
mild vs resp. ail. &  & 66/25 &  & 90.1 &  & 2.146e-09 \\
asymptomatic vs healthy &  & 16/275 &  & 77.2 &  & 1.293e-04 \\
asymptomatic vs resp. ail. &  & 16/25 &  & 62.8 &  & \textbf{0.089} \\
\cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(l){5-7}
\textbf{Prevalence(COVID:Non-COVID)} &  &  &  &  &  &  \\
1:3 &  & 100/300 &  & 92.1 &  & 1.019e-36 \\
1:2.5 &  & 100/250 &  & 92.6 &  & 7.734e-36 \\
1:2 &  & 100/200 &  & 91.7 &  & 2.650e-32 \\
1:1.5 &  & 100/150 &  & 91.3 &  & 1.032e-28 \\
1:1 &  & 100/100 &  & 93.5 &  & 1.232e-26 \\ \bottomrule
\end{tabular}
}
\caption{Description of the subject categories used in analysis.}
\label{tab:bias_analysis}
\end{table}

==> table_classifier.tex <==
\begin{table*}[]
% \rowcolors{2}{white}{gray!10}
\begin{tabular}{p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1cm}p{1cm}p{0.8cm}p{0.8cm}p{0.8cm}p{2cm}}
\hline
% \rowcolor[HTML]{9B9B9B} 
\textbf{Task} & \bf Breathing-deep &\bf Breathing-shallow & \bf Cough-heavy & \bf Cough-shallow & \bf Counting-fast  & \bf Counting-normal & \bf Vowel-[\ae] & \bf Vowel-[e] & \bf Vowel-[o] & \bf Fusion (Sensitivity at 95\% Specificity)\\ \hline
    \textbf{Omi-Del}      &       79.9      &     73.4        & 65.2  &   65.7  & 81.4  &  79.8 &  73.0 & 75.3  &  77.9 &  89.0 (52.4)   \\ \hline
    \textbf{Del-H}       &      73.3       &     70.1        & 72.2  &  75.0   & 81.3   & 80.5  & 70.9  & 70.3  & 71.1 & 88.3 (68.6)\\ \hline
     \textbf{Omi-H}      &     80.2        &     76.9        & 81.2  &   83.7  &  84.0 & 82.1  & 75.8  & 79.5  & 74.9  & 93.1 (71.4) \\ \hline
     \textbf{Pos-H}       &      76.1       &    74.4         & 76.7  &  80.1   & 83.4  & 82.0  & 75.4  & 76.6  &  75.0 & 90.5 (71.4) \\ \hline
\end{tabular}
\caption{Depiction of AUC for different classification tasks on the held out test set.}
\label{test_auc_table}
\vspace{-0.3in} 
\end{table*}


==> table_classifier_perfm_CI.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sample\\ name\end{tabular}}} &  & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sample\\ description\end{tabular}}} &  & \multicolumn{11}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Classifier performance on test set\\ (AUC \%)\end{tabular}}} \\ \cmidrule(l){5-15} 
 &  &  &  & \textbf{LR} &  & \textbf{RF} &  & \textbf{MLP} &  & \textbf{BLSTM} &  & \textbf{Transformer} \\ \midrule
Breathing &  & breathing-shallow &  & 69.9(64.9-74.5) &  & 76.6(71.7-80.9) &  & 78.6(74.2-82.8) &  & 77.9(73.5-81.9) &  & 78.1(73.8-82.1)  \\
 &  & breathing-deep &  & 68.7(63.6-73.7) &  & 74.0(68.5-78.5) &  & 74.5(69.4-78.8) &  & 75.7(71.0-80.2) &  & 76.7(71.9-81.2) \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{2}{*}{Cough} &  & cough-shallow &  & 73.6(68.6-77.9) &  & 77.1(72.4-81.2) &  & 76.8(72.0-81.1) &  & 76.6(71.7-80.8) &  & 75.5(70.8-79.7) \\
 &  & cough-heavy &  & 74.3(69.5-78.5) &  & 79.3(74.9-83.2) &  & 78.6(74.3-82.5) &  & 79.8(75.3-83.9) &  & 79.4(75.1-83.3)  \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Vowel\\ phonation\end{tabular}} &  & vowel-[u] &  & 70.0(65.1-74.5) &  & 75.7(71.3-80.0) &  & 73.2(68.5-77.5) &  & 73.6(68.4-78.6) &  & 74.9(69.9-79.6) \\
 &  & vowel-[i] &  & 69.4(64.5-74.1) &  & 74.3(69.2-79.0) &  & 69.6(64.0-74.3) &  & 77.3(73.1-81.9) &  & 77.5(73.3-81.9)  \\
 &  & vowel-[ae] &  & 71.1(66.4-75.6) &  & 77.3(72.9-81.4) &  & 70.5(65.4-75.0) &  & 79.3(74.5-83.4) &  & 78.6(74.0-82.6)  \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{2}{*}{Speech} &  & Counting normal &  & 69.4(64.5-73.9) &  & 76.0(71.1-80.2) &  & 75.7(71.1-80.0) &  & 80.8(76.6-84.7) &  & 80.1(75.7-83.8)  \\
 &  & Counting fast &  & 71.7(67.3-76.2) &  & 75.7(71.4-79.9) &  & 73.7(68.5-78.3) &  & 79.4(74.5-83.6) &  & 79.3(74.5-83.6) \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\begin{tabular}[c]{@{}l@{}}Sound\\ fusion\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Joint inference\\ using all sound\\ categories\end{tabular} &  & 73.9(69.1-78.2) &  & 78.9(74.4-82.6) &  & 76.2(71.4-80.6) &  & 84.1(80.1-87.8) &  & 84.1(80.2-87.7) \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\begin{tabular}[c]{@{}l@{}}Sound plus\\ symptom\\ fusion\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Joint inference\\ using all sound categories \\ plus symptom\end{tabular} &  & 89.2(85.8-92.1) &  & 91.2(88.2-93.8) &  & 90.1(86.9-93.0) &  & 92.1(89.3-94.4) &  & 92.0(89.2-94.1)  \\ \bottomrule
\end{tabular}
}
\caption{Description of binary classification performance for various classifier models (logistic regression (LR), random forest (RF), multi-layer perceptron (MLP), bi-directional long short-term memory (BLSTM) and transformer) on the different types of audio sample categories. A decision tree model is also trained for symptom based COVID classification with test set performance of $84.9\%$($81.0\%$-$88.5\%$). The sound plus symptom fusion results are obtained by combining the scores from all the sound classifiers with symptom based classifier scores.}
\label{tab:classification_results}
\end{table*}

==> table_classifier_perfm_std.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sample\\ name\end{tabular}}} &  & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sample\\ description\end{tabular}}} &  & \multicolumn{11}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Classifier performance on test set\\ (AUC \%)\end{tabular}}} \\ \cmidrule(l){5-15} 
 &  &  &  & \textbf{LR} &  & \textbf{RF} &  & \textbf{MLP} &  & \textbf{BLSTM} &  & \textbf{Transformer} &  & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ tree\end{tabular}}} \\ \midrule
Breathing &  & breathing-shallow &  & 69.9 [$\pm$3.0] &  & 76.6 [$\pm$2.8] &  & 78.6 [$\pm$2.6] &  & 77.9 [$\pm$2.6] &  & 78.1 [$\pm$2.5] &  & NA \\
 &  & breathing-deep &  & 68.7 [$\pm$3.0] &  & 74.0 [$\pm$3.0] &  & 74.5 [$\pm$2.9] &  & 75.7 [$\pm$2.9] &  & 76.7 [$\pm$2.8] &  & NA \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{2}{*}{Cough} &  & cough-shallow &  & 73.6 [$\pm$2.8] &  & 77.1 [$\pm$2.7] &  & 76.8 [$\pm$2.7] &  & 76.6 [$\pm$2.8] &  & 75.5 [$\pm$2.7] &  & NA \\
 &  & cough-heavy &  & 74.3 [$\pm$2.7] &  & 79.3 [$\pm$2.5] &  & 78.6 [$\pm$2.5] &  & 79.8 [$\pm$2.6] &  & 79.4 [$\pm$2.5] &  & NA \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Vowel\\ phonation\end{tabular}} &  & vowel-[u] &  & 70.0 [$\pm$2.9] &  & 75.7 [$\pm$2.6] &  & 73.2 [$\pm$2.7] &  & 73.6 [$\pm$3.1] &  & 74.9 [$\pm$3.0] &  & NA \\
 &  & vowel-[i] &  & 69.4 [$\pm$2.9] &  & 74.3 [$\pm$2.9] &  & 69.6 [$\pm$3.1] &  & 77.3 [$\pm$2.7] &  & 77.5 [$\pm$2.6] &  & NA \\
 &  & vowel-[ae] &  & 71.1 [$\pm$2.8] &  & 77.3 [$\pm$2.7] &  & 70.5 [$\pm$2.9] &  & 79.3 [$\pm$2.6] &  & 78.6 [$\pm$2.6] &  & NA \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\multirow{2}{*}{Speech} &  & Counting normal &  & 69.4 [$\pm$2.9] &  & 76.0 [$\pm$2.8] &  & 75.7 [$\pm$2.7] &  & 80.8 [$\pm$2.4] &  & 80.1 [$\pm$2.5] &  & NA \\
 &  & Counting fast &  & 71.7 [$\pm$2.7] &  & 75.7 [$\pm$2.7] &  & 73.7 [$\pm$2.9] &  & 79.4 [$\pm$2.7] &  & 79.3 [$\pm$2.7] &  & NA \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\begin{tabular}[c]{@{}l@{}}Sound\\ fusion\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Joint inferencing\\ using all sound\\ categories\end{tabular} &  & 73.9 [$\pm$2.8] &  & 78.9 [$\pm$2.6] &  & 76.2 [$\pm$2.8] &  & 84.1 [$\pm$2.3] &  & 84.1 [$\pm$2.3] &  & NA \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
Symptom &  & \begin{tabular}[c]{@{}l@{}}Health symptoms\\ (list here?)\end{tabular} &  & NA &  & NA &  & NA &  & NA &  & NA &  & 84.9 [$\pm$2.3] \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(lr){11-11} \cmidrule(lr){13-13} \cmidrule(l){15-15} 
\multicolumn{15}{l}{} \\
\begin{tabular}[c]{@{}l@{}}Sound plus\\ symptom\\ fusion\end{tabular} &  & \begin{tabular}[c]{@{}l@{}}Joint inferencing\\ using sound fusion\\ plus symptom\end{tabular} &  & 89.2 [$\pm$1.9] &  & 91.2 [$\pm$1.7] &  & 90.1 [$\pm$1.9] &  & 92.1 [$\pm$1.5] &  & 92.0 [$\pm$1.5] &  & NA \\ \bottomrule
\end{tabular}
}
\caption{Description of binary classification performance.}
\label{tab:classification_results}
\end{table*}

==> table_fusion_weights.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{ll|lcllc}
\hline
\textbf{Task}     &  &  & \textbf{sound-fusion} &  &  & \textbf{sound+symptom fusion} \\ \cline{1-1} \cline{4-4} \cline{7-7} 
breathing-shallow &  &  & 0.111                 &  &  & 0.006                         \\
breathing-deep    &  &  & 0.111                 &  &  & 0.039                         \\
cough-shallow     &  &  & 0.111                 &  &  & 0.023                         \\
cough-heavy       &  &  & 0.111                 &  &  & 0.075                         \\
vowel-o           &  &  & 0.111                 &  &  & 0.121                         \\
vowel-e           &  &  & 0.111                 &  &  & 0.001                         \\
vowel-a           &  &  & 0.111                 &  &  & 0.110                         \\
counting-normal   &  &  & 0.111                 &  &  & 0.250                         \\
counting-fast     &  &  & 0.111                 &  &  & 0.027                         \\
symptom           &  &  & -                     &  &  & 0.347                         \\ \hline
\end{tabular}

\caption{Optimum values of $\alpha_i$'s for fusion.}
\label{tab:weights_fusion}
\end{table}

==> table_health_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}lclclcrlrcr@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Subject\\ Category\end{tabular}} & \textbf{} & \textbf{\begin{tabular}[c]{@{}l@{}}Subject\\ sub-\\ category\end{tabular}} & \textbf{} & \textbf{Health status description} & \textbf{} & \multicolumn{5}{c}{\textbf{Subject count}} \\ \cmidrule(r){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(l){7-11} 
 &  &  &  &  &  & Train &  & Val &  & Test \\ \cmidrule(lr){7-7} \cmidrule(lr){9-9} \cmidrule(l){11-11} 
COVID &  & Asymp &  & \begin{tabular}[c]{@{}l@{}}COVID-19 positive status\\with no symptoms \end{tabular}&  & 42 &  & 10 &  & 16 \\\cmidrule(l){5-11}
 &  & Mild &  & \begin{tabular}[c]{@{}l@{}}COVID-19 positive status\\with mild symptoms \end{tabular}&  & 161 &  & 40 &  & 66 \\\cmidrule(l){5-11}
 &  & Moderate &  & \begin{tabular}[c]{@{}l@{}}COVID-19 positive status\\with moderate symptoms\end{tabular} &  & 42 &  & 11 &  & 18 \\ \midrule
\multicolumn{11}{l}{} \\
\begin{tabular}[c]{@{}l@{}}Non-\\ COVID\end{tabular} &  & Healthy &  & \begin{tabular}[c]{@{}l@{}}COVID-19 negative status with \\ no respiratory-ailments,\\ and without COVID-like symptoms\end{tabular} &  & 602 &  & 156 &  & 243 \\ \cmidrule(l){5-11} 
 &  & Resp. ail &  & \begin{tabular}[c]{@{}l@{}}COVID-19 negative status with \\  pre-existing respiratory\\ ailments including asthma,\\ pneumonia, or chronic lung disease\end{tabular} &  & 59 &  & 15 &  & 25 \\ \cmidrule(l){5-11} 
 &  & Symp &  & \begin{tabular}[c]{@{}l@{}} COVID-19 negative status with\\ no respiratory ailments but\\ has one or more COVID-19-like\\ symptoms such as cough, cold, fever,\\ loss of smell or muscle fatigue\end{tabular} &  & 58 &  & 8 &  & 32 \\ \bottomrule
\end{tabular}
\caption{Description of the subject categories and the respective counts used in analysis.}
\label{tab:data-partitions}
\end{table}

==> table_hyperparameters.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c|c|c}
    \hline 
    \textbf{Model}     &  \textbf{Hyper-parameter} & \textbf{Value}\\ \hline 
     \multirow{3}{*}{LR}    & $l_2$ regularization strength  & 100 \\ 
                            & optimizer & 'liblinear'\\
                            & maximum iterations    & 40\\
    \hline 
    \multirow{2}{*}{Decison Tree}    & criterion  & 'gini' \\
                                    & minimun samples for node split & 25\\
    \hline 
    \multirow{2}{*}{RF}    & estimators  & 20 \\ 
                            & impurity criterion & 'gini'\\
                            
     \hline 
     \multirow{4}{*}{MLP}    & hidden layers  & 1 \\ 
                            & hidden layer units  & 20 \\ 
                            & hidden layer activation & Tanh \\
                            & learning-rate & 0.001 \\
     \hline 
     \multirow{6}{*}{BLSTM}   & layers & 2\\
                            & encoder units & 128\\
                            & dropout & 0.1\\
                            & classifier units & 64\\
                            & classifier activation & Tanh\\
                            & classifier dropout & 0.1\\
     \hline 
     \multirow{7}{*}{Transformer}   & attention heads & 8\\
                            & layers & 1\\
                            & encoder units & 1024\\
                            & dropout & 0.1\\
                            & classifier units & 64\\
                            & classifier activation & Tanh\\
                            & classifier dropout & 0.1\\
     \hline 
     \multirow{1}{*}{Fusion}   & alphas & $\textbf{1}_{Kx1}$\\
     \hline 
    \end{tabular}
    \caption{The different models and hyper-parameters used for the classification.}
    \label{tab:hyper-parameters}
\end{table}

==> table_hyperparameters_BLSTM.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c|c|c}
    \hline 
    \textbf{Model}     &  \textbf{Hyper-parameter} & \textbf{Value}\\ \hline
     \multirow{6}{*}{BLSTM}   & layers & 2\\
                            & encoder units & 128\\
                            & dropout & 0.3\\
                            & classifier units & 16\\
                            & classifier activation & Tanh\\
                            & classifier dropout & 0.3\\
     \hline
     \multirow{1}{*}{Fusion}   & alphas & $\textbf{1}_{Kx1}$\\
     \hline 
    \end{tabular}
    \caption{The hyper-parameters used for the BLSTM classifier.}
    \label{tab:hyper-parameters-blstm}
\end{table}

==> table_metadata.tex <==
\begin{table}[]
\centering
\begin{tabular}{llrlrrr}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Coswara\\ Dataset\end{tabular}} &  & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}No\\ COVID-19\end{tabular}}} &  & \multicolumn{1}{c}{\textbf{COVID-19}} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Recovered\\ from\\ COVID-19\end{tabular}}} \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} 
\textbf{Subject} &  &  &  & \multicolumn{1}{c}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{} \\
Count &  & 1819 &  & 674  &  & 142  \\ \cline{1-1} \cline{3-7} 
\textbf{Sex} &  &  &  &  &  &  \\
Male &  & 1334 (73.3\%) &  & 409 (60.7\%) &  & 76 (53.5\%) \\
Female &  & 485 (26.7\%) &  & 264 (39.3\%) &  & 66 (46.5\%) \\ \cline{1-1} \cline{3-7} 
\textbf{Age} &  &  &  &  &  &  \\
15-30 &  & 934 (51.3\%) &  & 264 (39.2\%) &  & 64 (45.1\%) \\
30-45 &  & 554 (30.5\%) &  & 175 (26\%) &  & 40 (28.2\%) \\
45-60 &  & 261 (14.3\%) &  & 153 (22.7\%) &  & 28 (19.7\%) \\
60-90 &  & 70 (3.9\%) &  & 82 (12.1\%) &  & 10 (7\%) \\ \cline{1-1} \cline{3-7} 
\textbf{\begin{tabular}[c]{@{}l@{}}Indian \\ Province\end{tabular}} &  &  &  &  &  &  \\
Karnataka &  & 654 (36\%) &  & 322 (47.8\%) &  & 70 (49.3\%) \\
Tamil Nadu &  & 206 (11.3\%) &  & 247 (36.6\%) &  & 42 (29.6\%) \\
Maharashtra &  & 182 (10\%) &  & 42 (6.2\%) &  & 11 (7.7\%) \\
Kerala &  & 63 (3.5\%) &  & 17 (2.5\%) &  & 2 (1.4\%) \\
Others &  & 507 (27.9\%) &  & 34 (5\%) &  & 12 (8.5\%) \\ \hline
\end{tabular}

\caption{The demographic information of subjects in the Coswara dataset. The numbers correspond to human subject count.}
\label{table_dataset_description}
\vspace{-0.2in}
\end{table}

==> table_metadata_description.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{|p{2cm} |p{6cm}|}
\hline
\textbf{Field Name}       & \textbf{Description}                                                                                                               \\
\hline
id               & User ID                                                                                                                   \\
a                & Age (number)                                                                                                              \\
covid\_status    & Health status (e.g. : positive\_mild, healthy,etc.)                                                                       \\
record\_date     & Date when the user recorded and submitted the samples                                                                     \\
ep               & Proficient in English (y/n)                                                                                               \\
g                & Gender (male/female/other)                                                                                                \\
l\_c             & Country                                                                                                                   \\
l\_l             & Locality                                                                                                                  \\
l\_s             & State                                                                                                                     \\
rU               & Returning User (y/n)                                                                                                      \\
asthma           & Asthma (True/False)                                                                                                       \\
cough            & Cough (True/False)                                                                                                        \\
smoker           & Smoker (True/False)                                                                                                       \\
test\_status     & Status of COVID Test (p-\textgreater{}Positive, n-\textgreater{}Negative, na-\textgreater Not taken Test)                 \\
ht               & Hypertension (True/False)                                                                                                 \\
cold             & Cold (True/False)                                                                                                         \\
diabetes         & Diabetes (True/False)                                                                                                     \\
diarrhoea        & Diarrheoa  (True/False)                                                                                                   \\
um               & Using Mask (y/n)                                                                                                          \\
ihd              & Ischemic Heart Disease (True/False)                                                                                       \\
bd               & Breathing Difficulties (True/False)                                                                                       \\
st               & Sore Throat (True/False)                                                                                                  \\
fever            & Fever (True/False)                                                                                                        \\
ftg              & Fatigue (True/False)                                                                                                      \\
mp               & Muscle Pain (True/False)                                                                                                  \\
loss\_of\_smell  & Loss of Smell \& Taste (True/False)                                                                                       \\
cld              & Chronic Lung Disease (True/False)                                                                                         \\
pneumonia        & Pneumonia (True/False)                                                                                                    \\
ctScan           & CT-Scan (y/n if the user has taken a test)                                                                                \\
testType         & Type of test (RAT/RT-PCR)                                                                                                 \\
test\_date       & Date of COVID Test (if taken)                                                                                             \\
vacc             & Vaccination status (y-\textgreater{}both doses, p-\textgreater{}one dose(partially vaccinated), n-\textgreater{}no doses) \\
ctDate           & Date of CT-Scan                                                                                                           \\
ctScore          & CT-Score                                                                                                                  \\
others\_resp     & Respiratory illnesses other than the listed ones (True/False)                                                             \\
others\_preexist & Pre-existing conditions other than the listed ones (True/False)     \\                            \hline
\end{tabular}

\caption{Description of metadata collected along with the abbreviation of the metadata.}
\label{tab:metadata_description}
\end{table}

==> table_other_datasets.tex <==


\begin{table*}[t!]
\resizebox{\textwidth}{!}
{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lllllllccccclclccllllll}
\hline
\vspace{0.1in}
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Dataset\\ Name\end{tabular}}} & \textbf{}            & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sound data\end{tabular}}}         & \textbf{} &  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Sound\\ samples\\ per\\ subject\end{tabular}}} & \textbf{} & \multirow{2}{*}{{\textbf{\begin{tabular}[c]{@{}l@{}}Access\\ and\\ location\end{tabular}}}}                    & \textbf{} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Uncompressed\\audio file\\ \end{tabular}}} & \textbf{}                     & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Manual\\audio quality\\ validation \end{tabular}}} & \textbf{}            & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}COVID-19\\ screening\\ tool \\ developed\end{tabular}}} & \textbf{}            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Meta-data}}}                                                             & \textbf{}            & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Pre-existing\\ respiratory\\ condition\\ recorded \end{tabular}}} & \textbf{}            & \multicolumn{5}{c}{\textbf{Subject count}}                                                                                                                                                                              \\ \cline{19-23} 
 & \multicolumn{1}{c}{} &                                                                                      &  &                                                                                                   & \textbf{}                     &                                  & \textbf{}                     &                                                                                         & \textbf{}                     &                                                                                              &                      &                                                                                                           & \textbf{}            & \multicolumn{1}{c}{}                                                                                                & \textbf{}            &                                                                                                      & \textbf{}            & \textbf{\begin{tabular}[c]{@{}l@{}}non-\\ COVID-19\end{tabular}} & \textbf{}            & \textbf{COVID-19}         & \textbf{}            & \textbf{\begin{tabular}[c]{@{}l@{}}Recovered\\ from\\ COVID-19\end{tabular}} \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} \cline{11-11} \cline{13-13} \cline{15-15} \cline{17-17} \cline{19-19} \cline{21-21} \cline{23-23} 
 &                      &                                                                                      &  &                                                                                                   &                               &                                  &                               &                                                                                         &                               &                                                                                              &                      &                                                                                                           & \multicolumn{1}{l}{} &                                                                                                                     & \multicolumn{1}{l}{} &                                                                                                      & \multicolumn{1}{l}{} &                                                                &                      &                           &                      &                                                                              \\
\begin{tabular}[c]{@{}l@{}}COUGHVID\\ \cite{orlandic2020coughvid}\end{tabular}                             &                      & Cough                                                                                &  & 1                                                                                                 & \multicolumn{1}{c}{}          & \begin{tabular}[c]{@{}l@{}}Open\\ Europe and\\ beyond\end{tabular}                             & \multicolumn{1}{c}{}          & $\times $                                                                                     & \multicolumn{1}{c}{}          & $\times$                                                                                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\times$}                                                                                    &                      & \begin{tabular}[c]{@{}l@{}}Gender\\ Age\\ Other diseases\\ Symptoms\\ Location\end{tabular}                         &                      & $\times$                                                                                                &                      & \multicolumn{1}{l}{26395}                                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{1155}  & \multicolumn{1}{r}{} & \multicolumn{1}{l}{None}                                                     \\ \cline{1-1} \cline{3-23} 
 &                      &                                                                                      &  &                                                                                                   &                               &                                  &                               &                                                                                         &                               &                                                                                              &                      &                                                                                                           & \multicolumn{1}{l}{} &                                                                                                                     & \multicolumn{1}{l}{} &                                                                                                      & \multicolumn{1}{l}{} &                                                                &                      &                           &                      &                                                                              \\
\begin{tabular}[c]{@{}l@{}}COVID-19\\ Sounds\\\cite{han2022sounds}\end{tabular}                    &                      & \begin{tabular}[c]{@{}l@{}}Cough\\ Breathing\\ Speech\end{tabular}                   &  & 3                                                                                                 & \multicolumn{1}{c}{}          & \begin{tabular}[c]{@{}l@{}}On request\\ \textcolor{markChanges}{Europe, UK,}\\\textcolor{markChanges}{USA}\\ \textcolor{markChanges}{and beyond}\end{tabular}                          & \multicolumn{1}{c}{}          & $\times$                                                                                      & \multicolumn{1}{c}{}          & $\times$                                                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\times$}                                                                                    &                      & \begin{tabular}[c]{@{}l@{}}Gender\\ Medical history\\ Symptoms\\ Hospitalization\end{tabular}                       &                      & $\times$                                                                                                     &                      & \multicolumn{1}{l}{6450}                                       & \multicolumn{1}{r}{} & \multicolumn{1}{l}{2106}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{None}                                                     \\ \cline{1-1} \cline{3-23} 
 &                      &                                                                                      &  &                                                                                                   &                               &                                  &                               &                                                                                         &                               &                                                                                              &                      &                                                                                                           & \multicolumn{1}{l}{} &                                                                                                                     & \multicolumn{1}{l}{} &                                                                                                      & \multicolumn{1}{l}{} &                                                                &                      &                           &                      &                                                                              \\
\begin{tabular}[c]{@{}l@{}}Tos\\ COVID-19\\\cite{pizzo2021iatos}\end{tabular}                       &                      & Cough                                                                                &  & 1                                                                                                 & \multicolumn{1}{c}{\textbf{}} & \begin{tabular}[c]{@{}l@{}}Open\\ Argentina \end{tabular}                             & \multicolumn{1}{c}{\textbf{}} & $\times$                                                                                     & \multicolumn{1}{c}{\textbf{}} & $\times$                                                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\times$}                                                                                    & \textbf{}            & \begin{tabular}[c]{@{}l@{}}Gender\\ Age\\ Symptoms\\ Location\end{tabular}                                          & \textbf{}            & $\times$                                                                                             & \textbf{}            & \multicolumn{1}{l}{125183}                                     & \multicolumn{1}{r}{} & \multicolumn{1}{l}{21197} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{None}                                                     \\ \cline{1-1} \cline{3-23} 
 &                      &                                                                                      &  &                                                                                                   &                               &                                  &                               &                                                                                         &                               &                                                                                              &                      &                                                                                                           & \multicolumn{1}{l}{} &                                                                                                                     & \multicolumn{1}{l}{} &                                                                                                      & \multicolumn{1}{l}{} &                                                                &                      &                           &                      &                                                                              \\
\begin{tabular}[c]{@{}l@{}}Coswara\\ (This work)\end{tabular}                   &                      & \begin{tabular}[c]{@{}l@{}}Cough (2 types)\\ Breathing (2 types)\\ Vowel phonation (3 types)\\ Speech (2 types)\end{tabular} &  & 9                                                                                                 & \multicolumn{1}{c}{}          & \begin{tabular}[c]{@{}l@{}}Open\\ India and\\ beyond\end{tabular}                             & \multicolumn{1}{c}{}          & $\checkmark$                                                                                     & \multicolumn{1}{c}{}          &     $\checkmark$                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}                                                                                   &                      & \begin{tabular}[c]{@{}l@{}}Gender\\ Age\\ Country\\ Symptoms\\ Other ailments\\ Vaccination\\ and more\end{tabular} &                      & $\checkmark$                                                                                                &                      & \multicolumn{1}{l}{1819}                                       & \multicolumn{1}{c}{} & \multicolumn{1}{l}{674}   &                      & \multicolumn{1}{l}{142}                                                      \\ \hline
\end{tabular}
}
\caption{List of publicly accessible COVID-19 related respiratory sound datasets.}
\label{tab:other_datasets}
\vspace{-0.2in}
\end{table*}


% \begin{table*}[t!]
% %\begin{fullwidth}
% \centering
% % \rowcolors{2}{white}{gray!10}
% \begin{center} 
% \begin{tabular}{  p{3.5cm} p{4cm}  p{2cm} p{ 2.5cm}  p{3.5cm} }
% \hline
% \textbf{Name} & \textbf{Category} & \textbf{Access} & \textbf{Positive/Negative} & \textbf{Method}       \\ \hline
%  COUGHVID~\cite{orlandic2020coughvid} & Cough & Public & 1155/26395 & Crowdsourced \\ 
%   Virufy~\cite{virufy_set}& Cough & Public & 48/73 & Hospital \\ 
%  NoCoCoDa~\cite{nocoda}  & Cough & On request & 13/NA & YouTube\\
  
%  COVID-19 Sounds~\cite{brown2020exploring}& Cough, Breathing, Speech & On request & 2106/6450 & Crowdsourced\\
 
%   COVID-19 Cough~\cite{ponomarchuk2021project}& Cough & public & 682/642 & Partial clinical validation\\
 
%   Tos COVID-19~\cite{pizzo2021iatos}& Cough & public & 2926/2941 & clinical validation\\
%   \hline \hline 
%  This work -- \textbf{Coswara}~\cite{sharma2020coswara} & Breathing, Cough, Vowels, Speech, Symptoms & Public & 681/1590 & Partial clinical validation \\ \hline
% \end{tabular}

% \caption{A list of COVID-19 acoustics accessible datasets.\textcolor{red}{nocoda citation, symptoms daataset, tool release}
% % \textcolor{red}{Need to double check the numbers in this table  }
% }
% \end{center} 
% \label{table:literature_review}
% %\end{fullwidth}
% \end{table*}

==> table_severity_audio_fusion.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}
{
\begin{tabular}{l|c|c|c}
\hline
                    & \textbf{Pos-moderate} & \textbf{Pos-mild} & \textbf{Pos-asymp} \\ \hline
\textbf{healthy}    & 85.2 (75.4-93.3)      & 87.1 (82.8-91.1)  & 81.7 (72.6-89.9)   \\
\textbf{symp}       & 70.5 (57.2-82.5)      & 73.9 (64.3-83.0)  & 64.4 (51.1-78.8)   \\
\textbf{Resp. ail.} & 83.2 (71.3-93.1)      & 83.6 (75.9-90.4)  & 76.6 (63.4-88.5)   \\ \hline
\end{tabular}
}
\caption{Performance of audio-fusion classifier for different COVID and Non-COVID groups}
\label{tab:covid_severity_audio_fusion}
\end{table}

==> table_severity_audio_fusion_v2.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}
{
\begin{tabular}{lllcll}
\hline
                           &  & \textbf{\begin{tabular}[c]{@{}l@{}}Count\\ COVID/\\ Non-COVID\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}AUC\\ (\%)\end{tabular}} &  & \multicolumn{1}{c}{\textbf{p value}}  \\ \hline
Pos-moderate vs healthy    &  & 18/243                                                                      & 85.2 (75.4-93.3)                                            &  & \multicolumn{1}{c}{0.252}             \\
Pos-moderate vs symp       &  & 18/32                                                                       & 70.5 (57.2-82.5)                                            &  & \multicolumn{1}{c}{p\textless{}0.050} \\
Pos-moderate vs Resp. ail. &  & 18/25                                                                       & 83.2 (71.3-93.1)                                            &  & \multicolumn{1}{c}{0.253}             \\ \cline{1-1} \cline{3-4} \cline{6-6} 
Pos-mild vs healthy        &  & 66/243                                                                      & 87.1 (82.8-91.1)                                            &  & 0.200                                 \\
Pos-mild vs symp           &  & 66/32                                                                       & 73.9 (64.3-83.0)                                            &  & p\textless{}0.050                     \\
Pos-mild vs Resp. ail.     &  & 66/25                                                                       & 83.6 (75.9-90.4)                                            &  & 0.200                                 \\ \cline{1-1} \cline{3-4} \cline{6-6} 
Pos-asymp vs healthy       &  & 16/243                                                                      & 81.7 (72.6-89.9)                                            &  & 0.084                                 \\
Pos-asymp vs symp          &  & 16/32                                                                       & 64.4 (51.1-78.8)                                            &  & p\textless{}0.050                     \\
Pos-asymp vs Resp. ail.    &  & 16/25                                                                       & 76.6 (63.4-88.5)                                            &  & 0.084                                 \\ \hline
\end{tabular}
}
\caption{Performance of audio-fusion classifier for different COVID and Non-COVID groups}
\label{tab:covid_severity_audio_fusion_v2}
\end{table}
